Evaluating Interpolation and Extrapolation Performance of Neural Retrieval Models

A retrieval model should not only interpolate the training data but also extrapolate well to the queries that are different from the training data. While neural retrieval models have demonstrated impressive performance on ad-hoc search benchmarks, we still know little about how they perform in terms of interpolation and extrapolation. In this paper, we demonstrate the importance of separately evaluating the two capabilities of neural retrieval models. Firstly, we examine existing ad-hoc search benchmarks from the two perspectives. We investigate the distribution of training and test data and find a considerable overlap in query entities, query intent, and relevance labels. This finding implies that the evaluation on these test sets is biased toward interpolation and cannot accurately reflect the extrapolation capacity. Secondly, we propose a novel evaluation protocol to separately evaluate the interpolation and extrapolation performance on existing benchmark datasets. It resamples the training and test data based on query similarity and utilizes the resampled dataset for training and evaluation. Finally, we leverage the proposed evaluation protocol to comprehensively revisit a number of widely-adopted neural retrieval models. Results show models perform differently when moving from interpolation to extrapolation. For example, representation-based retrieval models perform almost as well as interaction-based retrieval models in terms of interpolation but not extrapolation. Therefore, it is necessary to separately evaluate both interpolation and extrapolation performance and the proposed resampling method serves as a simple yet effective evaluation tool for future IR studies.

==> correlation.tex <==
\subsection{Extrapolation vs. Generalization}
\label{sec:relation_domain_transfer}

After evaluating the extrapolation performance of existing ranking models, we investigate the relationship between extrapolation performance and another generalization capacity, i.e., domain transfer ability. Domain transfer tasks evaluate how well a ranking model performs in out-of-domain scenarios. For example, the model is trained on Web search data and is transferred to medical domains. It has drawn considerable attention from the neural IR community~\cite{thakur2021beir, xin2021zero, izacard2021towards, wang2021gpl}. 
To provide a deeper understanding of extrapolation evaluation, we investigate how benchmark extrapolation results correlate domain transfer ability~(\textbf{RQ3}).
In the following, we first introduce the current domain transfer tasks and then discuss the correlation.

\subsubsection{Domain Transfer and BEIR dataset} \mbox{}

Domain transfer is important for low-resource domains such as finance and medicine where supervision data is hard to obtain. It is difficult to directly train a neural ranking model in such domains because neural models are data-hungry. To resolve this problem, a model is trained in data-rich domains and is then directly used in the target domain.

Evaluating the domain transfer ability is hard and costly. To construct a meaningful and trustworthy domain transfer task, one should select a low-resource domain and the annotation should be complete. However, annotation is costly for many low-resource domains such as medicine and is even prohibited due to privacy restrictions. To make matters worse, evaluating retrieval models requires annotating a large candidate pool per query so that almost all relevant pairs are labeled. Otherwise, the top-ranked documents may be false negatives and the evaluation results are not trustworthy. Therefore, annotating such a dataset is expensive. 
On the contrary, our resampling strategies do not require a new dataset. We reuse the existing ad-hoc benchmarks~\cite{craswell2019overview, Craswell2020Overview}, which involve relatively comprehensive annotations. Researchers can easily test the extrapolation performance via retraining the models on the resampled training sets. 

%BEIR is an existing popular tool to evaluate domain transfer ability. It contains various retrieval datasets from different domains or tasks. The evaluation protocol is to test the zero-shot performance of ranking models. 
%Despite its popularity, it is worth mentioning that it has two problems. 
%First, the annotation of its datasets has strong lexical bias. The bias originates from the annotation pools, which are constructed by traditional lexical methods. Thus, the relevant documents not recalled by lexical methods become false negatives. The bias severely underestimates the performance of DR models because they do not utilize lexical matching signals and their top-ranked documents are always missing from the annotations~\cite{xin2021zero, thakur2021beir}. Therefore, BEIR is not suitable to compare models with and without lexical matching modules. 
%The second issue of BEIR is the inconsistent definitions of relevance. Some of the datasets in BEIR are not typical ad-hoc retrieval tasks. For example, some tasks are fact checking, argument retrieval, counter-argument retrieval, etc. Their definitions of relevance are different from that of ad-hoc search. 
%In contrast, our extrapolation evaluation has much less lexical bias due to relatively comprehensive annotations and the relevance definitions are consistent.


\subsubsection{Correlation Investigation} \mbox{}

After introducing the BEIR dataset, now we investigate the correlation between the extrapolation performance evaluated by resampling methods and the out-of-domain performance evaluated by the BEIR dataset. 
Note that BEIR is not perfect, i.e., lexical annotation bias and inconsistent definitions of relevance, as introduced in the previous section.
To alleviate the effect of lexical annotation bias, we only use dense retrieval models for correlation investigation so that no models take advantage of the bias. But it is worth pointing out that our evaluation methods based on the benchmark data do not have such bias and can evaluate models of other architectures. 
As for inconsistent definitions of relevance in BEIR, we decide to compute correlation with each dataset in BEIR instead of with the average performance of all BEIR datasets. We check the associated dataset paper if the correlation results are abnormal.
In the following, we first present the implementation details and then discuss the results.

%\subsubsection{Implementation} \mbox{}
%
%We train DR models using the resampled training data with different settings to acquire various models. We evaluate their interpolation and extrapolation performance on retrieval benchmarks~\cite{craswell2019overview, Craswell2020Overview}. We also evaluate the transfer performance using the BEIR dataset. Finally, we study the correlation between the interpolation/extrapolation performance and the transfer performance. 
%
%Additionally training many DR models may exceed our computational budget, but fortunately, we have trained many DR models in Section~\ref{sec:evaluate_extrapolation}. Therefore, we reuse these trained DR models and only need to evaluate the performance on the BEIR dataset.
%In Section~\ref{sec:evaluate_extrapolation}, ReSTrain samples three sizes of training data for each model setting. Thus, it produces many model variants and the computed correlation results are reliable. However, ReSTTest does not subsample the training data and the number of checkpoints is not enough for correlation computation. Therefore, we only compute the correlation between ReSTrain and BEIR dataset, but we believe the results also generalize to ReSTTest.
%
%The reused DR models are from Table~\ref{tab:compare_hard_distill_pretrain} and Table~\ref{tab:compare_pretrain}. In Table~\ref{tab:compare_hard_distill_pretrain}, we have trained models with hard negative mining and distillation. In Table~\ref{tab:compare_pretrain}, we have trained the models initialized by RoBERTa~\cite{liu2019roberta}, BERT~\cite{devlin2019bert}, ERNIE2.0~\cite{Sun2020ERNIE2A}, Condenser~\cite{gao2021condenser}, coCondenser-wiki~\cite{gao2021unsupervised}, and coCondenser-marco~\cite{gao2021unsupervised}. We reuse $8$ model settings in total. Considering that ReSTrain samples $3$ sizes of training set, i.e., $14k$, $45k$, and $200k$ training queries, for both interpolation and extrapolation, we reuse $48$ checkpoints of which half is trained on the interpolation training set and the other half is trained on the extrapolation training set. We evaluate their out-of-domain performance on BEIR and compute the spearman and kendall correlation results. Note that we exclude the randomly initialized DR model in Table~\ref{tab:compare_pretrain}. Since this weak model achieves the worst performance, including it simply increases the correlation numbers. But such an increase also hides the fact that the correlation with some BEIR datasets is extremely low. Therefore, we decide to exclude this model. 

    
\begin{table}[t]
    \small
    \caption{Ranking performance (NDCG@10) correlation between TREC-Covid and TREC DL. ReSTrain evaluates interpolation and extrapolation performance on TREC DL. More correlated results are marked bold except for very low correlation. Results suggest the extrapolation performance is substantially more correlated to transfer ability than interpolation. }
    \label{tab:correlation_coefficient}
    \begin{tabular}{ll|cc|cc}
    \toprule
    \multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{Domain}} & \multicolumn{2}{c|}{\textbf{Spearman}} & \multicolumn{2}{c}{\textbf{Kendall}} \\
    & & \textbf{Inter.} & \textbf{Extra.} & \textbf{Inter.} & \textbf{Extra.} \\ \midrule
    {TREC-Covid} 	& Bio-Medical	& 0.537 & \textbf{0.841} & 0.359 & \textbf{0.645} \\
    {NFCorpus} 		& Bio-Medical 	& 0.582 & \textbf{0.783} & 0.418 & \textbf{0.611} \\
    {NQ} 			& Wiki-QA		& 0.791 & \textbf{0.935} & 0.606 & \textbf{0.805} \\
    {HotpotQA} 		& Wiki-QA		& 0.579 & \textbf{0.836} & 0.416 & \textbf{0.635} \\
    {DBPedia} 		& Wiki-Entity	& 0.647 & \textbf{0.846} & 0.492 & \textbf{0.679} \\
    {CQADupS.}		& StackEx. Query& 0.577 & \textbf{0.902} & 0.403 & \textbf{0.730} \\
    {Quora} 		& Quora	Query	& 0.655 & \textbf{0.823} & 0.493 & \textbf{0.647} \\
    {SciDocs} 		& Sci Citation	& 0.595 & \textbf{0.724} & 0.440 & \textbf{0.546} \\
    {SciFact} 		& Sci Fact-check& 0.603 & \textbf{0.793} & 0.453 & \textbf{0.611} \\
    {Arguana} 		& Counter-argu.	& \textbf{0.612} & 0.504 & \textbf{0.435} & 0.375 \\
	{FiQA} 			& Finance-QA	& 0.273 & 0.283 & 0.223 & 0.199 \\
	{FEVER} 		& Wiki Fact-check& -0.284 & -0.175 & -0.179 & -0.142 \\
	{Climate-F.} 	& Wiki Fact-check& -0.515 & -0.352 & -0.419 & -0.260 \\
	{Touch{\'e}-2020} 	& Argument		& -0.307 & -0.410 & -0.216 & -0.278 \\
    \midrule
    \bottomrule
    \end{tabular}
    \end{table}
    
    
\begin{figure}[t]
	\subfloat[TREC-Covid vs. TREC DL interpolation]{\label{fig:correlation_inter_ndcg}\includegraphics[width=0.45\linewidth]{drawing/allset/allset-inter-ndcg}}   
	\hspace{5mm}
	\subfloat[TREC-Covid vs. TREC DL extrapolation]{\label{fig:correlation_extra_ndcg}\includegraphics[width=0.45\linewidth]{drawing/allset/allset-extra-ndcg}}  
	\caption{Ranking performance~(NDCG@10) on TREC-Covid~(y-axis) and TREC DL~(x-axis). Interpolation and extrapolation performances on TREC DL are measured with ReSTrain.}
	\label{fig:correlation_ndcg}
\end{figure}


\subsubsection{Discussion} \mbox{}

The correlation of ranking performance evaluated by ReSTrain or BEIR datasets is shown in Table~\ref{tab:correlation_coefficient}. 
For the majority of BEIR datasets, extrapolation performance on benchmarks is substantially more correlated to the out-of-domain performance. These datasets cover multiple domains, including bio-medicine~\cite{voorhees2021trec, boteva2016full}, wiki-QA~\cite{yang2018hotpotqa, kwiatkowski2019natural}, entity search~\cite{hasibi2017dbpedia}, duplicate question retrieval~\cite{hoogeveen2015cqadupstack}, citation prediction~\cite{cohan2020specter}, and science fact-checking~\cite{wadden2020fact}. 
Among these BEIR datasets, TREC-Covid~\cite{voorhees2021trec}, NQ~\cite{kwiatkowski2019natural}, and HotpotQA~\cite{yang2018hotpotqa} are widely adopted, and the evaluation results on them are assumed to be reliable. The strong correlation to these datasets is a trustworthy signal that extrapolation has the potential to reflect domain adaption ability. The results further verify the importance of evaluating extrapolation performance on benchmarks as the interpolation performance is much less consistent with the transfer performance.

To present the correlation more clearly, we plot interpolation-transfer and extrapolation-transfer relations in Figures~\ref{fig:correlation_inter_ndcg} and \ref{fig:correlation_extra_ndcg}, respectively. The x-axis shows the performance on the ad-hoc search benchmark~(TREC 19 \& 20 DL), and the y-axis shows the transfer performance~(TREC-Covid). We use the TREC-Covid~\cite{voorhees2021trec} dataset as a transfer example because it features a typical low-resource domain and its relevance definition is consistent with that of ad-hoc search. Previous work~\cite{xin2021zero} regards it as the most reliable dataset in BEIR. 
The two figures are consistent with the correlation results in Table~\ref{tab:correlation_coefficient}. The points in Figure~\ref{fig:correlation_extra_ndcg}  clearly follow an upward trend, whereas the points in Figure~\ref{fig:correlation_inter_ndcg} do not. The results suggest that if a model achieves good in-domain extrapolation performance, it is also very likely to achieve good out-of-domain transfer performance. 

%We also find abnormal results in the correlation analysis for some BEIR datasets. 
%Except for FiQA~\cite{maia2018WWW18OC} whose paper contains little information about how the dataset is constructed, we conjecture the abnormal results for the rest datasets are caused by inconsistent definitions of relevance.
%Concretely, Arguana~\cite{wachsmuth2018retrieval} and Touch{\'e}-2020~\cite{bondarenko2020OverviewOT} are both argument retrieval tasks. Arguana~\cite{wachsmuth2018retrieval} requires retrieving counterarguments that should have the opposite stance. Touch{\'e}-2020~\cite{bondarenko2020OverviewOT} requires retrieving arguments that help users engage in an argumentative conversation. 
%As for FEVER~\cite{thorne2018fever} and Climate-FEVER~\cite{diggelmann2020climate}, they require retrieving evidence that supports given claims. 
%The relevance definitions of the four datasets are different from the typical query-document relevance definitions in ad-hoc search.
%Note that another fact-checking dataset, SciFact~\cite{wadden2020fact}, is an exception: it has a strong correlation with benchmark performance. We find the claim-evidence pairs in this dataset are natural sentences and their cited papers. Therefore, it guarantees that the claims are representative of the evidence. In contrast, such relations do not exist in FEVER~\cite{thorne2018fever} and Climate-FEVER~\cite{diggelmann2020climate}. 










==> latex_tables/relation_label_query_overlap.tex <==
\begin{table}[t]
    \small
    \caption{Confusion matrix between label overlap and query intent overlap.}
    \label{tab:relation_label_query_overlap}
    \begin{tabular}{ll|cc}
    \toprule
    \multicolumn{2}{l|}{\multirow{2}{*}{\textbf{TREC 19 \& 20 DL}}} 
      & \multicolumn{2}{c}{\textbf{Query Intent}}   \\
    & & \textbf{Duplicate or Similar} & \textbf{Dissimilar}   \\
    \midrule
    \multirow{2}{*}{\textbf{Passage}}	
    	& {\textbf{Overlap}} 	& 59\% & 19\% \\
    	& {\textbf{No overlap}} & 9\% & 13\% \\
    \bottomrule
    \end{tabular}
    \end{table}
